Quantifying Interstellar Extinction at High Galactic Latitudes

A detailed map of the distribution of dust at high Galactic latitudes is essential for future cosmic microwave background (CMB) polarization experiments because the dust, while diffuse, remains a significant foreground in these regions. We develop a Bayesian model to identify a region of the Hertzsprung-Russell (HR) diagram suited to constrain the single-star extinction accurately at high Galactic latitudes. Using photometry from Gaia, 2MASS and ALLWISE, and parallax from Gaia, we employ nested sampling to fit the model to the data and analyse the posterior over stellar parameters for both synthetic and real data. Charting low variations in extinction is complex due to systematic errors and degeneracies between extinction and other stellar parameters. The systematic errors can be minimised by restricting our data to a region of the HR diagram where the stellar models are most accurate. Moreover, the degeneracies can be reduced by including astrophysical priors and spectroscopic constraints. We show that accounting for the measurement error of the data and the assumed inaccuracies of the stellar models are critical in accurately recovering small variations in extinction. We compare the posterior distribution for individual stars with spectroscopic stellar parameter estimates from LAMOST and Gaia ESO and illustrate the importance of estimating extinction and effective temperature as a joint solution.

==> old5_5.tex <==
\subsection{Dust Map Comparison}


We use a well-studied region and run our full model, including all necessary cuts, to derive a map of extinction and compare it with other dust maps.  We select a square region of width $3^\circ$ region centred on $l=104^\circ$ and $b=22.5^\circ$ which has been studied in \cite{Panopoulou_2019} by the PASIPHAE team \citep{tassis2018pasiphae}, where they show that the polarization signal is a tracer of two large clouds in the sightline, each at varying distances. Figure 1 in \cite{Panopoulou_2019} shows the H1 emission maps of the region.



{We query the Gaia database for stars within the square region defined above and cross-match with 2MASS and ALLWISE in the same manner as described in Section \ref{Data}. Moreover, we apply the recommended quality cuts described therein. We run our model to generate samples from the posterior distribution of each star in the sample. For each star, we use the posterior samples to calculate $\mathbb{E}[A_0]^{(i)}$ and $\text{Var}[A_0]^{(i)}$, the posterior mean and variance of extinction, respectively.}

{
We take the posterior mean extinction value for each star and carry out {a Gaussian filter to smooth the values spatially. This is done using a K-nearest neighbours algorithm search to find the $50$ nearest spatial neighbours of each point in the $(l,b)$ plane. Subsequently, we apply a Gaussian filter to compute the weighted average, where the variance of the Gaussian filter is given by $\sigma_i=\sqrt{\text{Var}[A_0]^{(i)}}$}. The explicit form of the Gaussian filter is $w(\delta l, \delta b,\sigma_i) = e^{-\frac{{\delta l}^2+\delta b^2}{0.1*2\sigma_i^2}}$, where $\delta l, \delta b$ correspond to the difference between the centre and a neighbour's Galactic longitude and latitude, respectively. Thus, for each star in the sample, we return a new value of extinction, which has been averaged spatially over nearby points. The Gaussian smoothing process is to validate our model against other surveys which use a similar smoothing algorithm. However, in future, we wish to extract dust information without assuming Gaussian correlation on the spatial distribution of dust.}


In Figure \ref{fig:full_maps} we display our dust map generated using a full solution (top-left plot) assuming an exponential prior on $A_0$ with {scale parameter} $d_A=0.2$. In the top-right plot, we show the HI emission map from \cite{Lenz_2017}. Moreover, we compare these dust maps with the Planck extinction map \citep{Planck} (bottom-left) and the Bayestar \citep{bayestar} dust map (bottom-right) for the same region.  {The numerical scale of each extinction map differs by a different constant for each map, we adjust the values of each map so that 0 corresponds to the minimum and 1 corresponds to the maximum extinction in each extinction map.} We calculate a residual between our dust map using the full solution and the other dust maps by finding the absolute difference $|\Delta A_0|$ for the scaled extinction at each point of the dust map. We display the residuals in Figure \ref{fig:residuals}.

We see there is a high correlation between our full solution dust map and the dust map generated by Bayestar. In particular the region of high extinction between $103.0^\circ<l<104.5^\circ$ at the bottom of our dust map is present in both maps (and indeed the other maps as well). Moreover, there is a correlation between our dust map and the Baystar dust map for regions of high extinction and low extinction. By looking at the residuals we see that there is a significant feature in the Planck map that is not present in the other maps. This is because the Planck map has been integrated to infinity, whereas our dust map and the Bayestar dust map both use radial distance and we have not probed distances to reach the cloud, which we know from \cite{Panopoulou_2019}. 

Another key feature of the dust clouds mentioned in \cite{Panopoulou_2019} is the circular type cloud bounded by $104^\circ<l<104.5 ^\circ$ and $22.05^\circ<b<23.0 ^\circ$, which can be seen vaguely in the Planck dust map. We note that our method shows some relatively low extinction in this region, but does not reproduce the same topology as the Planck map.

It is important to note that our dust maps have been generated using the mean value of the extinction posterior. {{It is reassuring to see a good agreement between our map and other surveys. However, this is a point of validation for us and to generate these dust maps we have smoothed over a lot of signal, be it artificial or real. We wish to have a methodology to probe single-star extinctions along a line-of-sight at high Galactic latitudes to generate accurate line-of-sight profiles to find fine variation in the ISM. Most extinction-based dust maps such as \cite{bayestar} look to chart large-scale structure in our Galaxy. We are interested in charting extinction over small sightlines, without performing any smoothing, to reflect the impact of the complex nature of dust on B mode detection.}}

Large regions of high extinction will appear as regions of high extinction provided there are enough background stars to probe the cloud. However, {due to spatial smoothing and taking single point estimates} regions of low extinction can give a relatively large mean value of the extinction too, generating artificial structure in the dust map. We can see this is particularly true in the case when we use photometry and parallax only. As these artificially large representations of the extinction get smoothed spatially, we generate false, artificial structures. Hence, to detect fine variation in the ISM, we will need to use the full posterior distribution of extinction.



\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/maps-2.png}
    \caption{Comparison between dust maps of a $3^\circ$ Region Centered at Galactic Coordinates $l=104^\circ$ and $b=22.5^\circ$, as studied by the PASIPHAE team in 2019. \protect\cite{Panopoulou_2019} have studied this region to show HI maps trace two different clouds at different distances. The top-left image is our dust map generated by smoothing over the posterior mean extinction using photometry, parallax and an effective temperature estimate. The top-right image shows the HI emission for the region. The bottom-left image shows the Planck dust map for the same region, and the bottom-right shows the Bayestar dust map for the same region. The topology of each dust map is complex due to smoothing effects.}
    \label{fig:full_maps}
\end{figure*}



\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/residuals.png}
    \caption{Comparison of the residuals between our full solution dust map and the other dust maps, for a $3^\circ$ Region Centered at Galactic Coordinates $l=104^\circ$ and $b=22.5^\circ$, as described in Figure \ref{fig:full_maps}. The hue is the absolute difference between the dust maps, scaled between 0 and 1. Here we see that there is significant agreement between our dust map and the Bayestar dust map. Moreover, by looking at the residuals, we can see the cloud in the bottom-left of the Planck dust map which we know is outside the region we have probed.}
    \label{fig:residuals}
\end{figure*}
